Patch redundancy in images: a statistical testing framework and some applications

In this work we introduce a statistical framework in order to analyze the spatial redundancy in natural images. This notion of spatial redundancy must be defined locally and thus we give some examples of functions (auto-similarity and template similarity) which, given one or two images, computes a similarity measurement between patches. Two patches are said to be similar if the similarity measurement is small enough. To derive a criterion for taking a decision on the similarity between two patches we present an a contrario model. Namely, two patches are said to be similar if the associated similarity measurement is unlikely to happen in a background model. Choosing Gaussian random fields as background models we derive non-asymptotic expressions for the probability distribution function of similarity measurements. We introduce a fast algorithm in order to assess redundancy in natural images and present applications in denoising, periodicity analysis and texture ranking.

==> shared_tex.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
%\usepackage{algorithmic}
\usepackage{pgfplots}
\usetikzlibrary{spy}
\usepackage{mathrsfs}
\input{header}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Testing redundancy in images: an a contrario framework}{V. De Bortoli, A. Desolneux, B. Galerne, A. Leclaire}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
% \title{Patch redundancy in images: a statistical testing framework and some applications \thanks{Submitted to the editors DATE.}}
\title{Patch redundancy in images: a statistical testing framework and some applications \thanks{Submitted to the editors DATE.}}


% Authors: full names plus addresses.
\author{Valentin De Bortoli\thanks{CMLA, ENS Cachan, CNRS, Université Paris-Saclay, 94235 Cachan, France
}
\and Agnès Desolneux\footnotemark[2]
\and Bruno Galerne\thanks{Institut Denis Poisson, Universit\'{e} d'Orléans, Universit\'{e} de Tours, CNRS}
\and Arthur Leclaire\thanks{Univ. Bordeaux, IMB, Bordeaux INP, CNRS, UMR 5251, F-33400 Talence, France.}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sim_fun.tex <==
\section{An a contrario framework for auto-similarity}
\label{sec:similarity functions}
% \subsection{Similarity functions}
% \label{sec:def_statistical_prop}
% In order to evaluate redundancy in images we first need to derive a criterion for comparing images. We propose to use similarity functions which take two images, or sub-images, as inputs.%  Before discussing the choice of function, or patch 
% domain, we must precise which images are going to be used to conduct the redundancy detection. 

% Indeed, when comparing sub-images, two cases can occur. We can compare a patch  with another patch extracted from the same image. We call this situation \textit{internal matching}. Applications can be found in denoising \cite{buades2005non} or inpainting \cite{criminisi2004region} where the information of the image itself is used to perform the image processing task. On the other hand, we can compare a patch with a patch extracted from another image. We call this situation \textit{template matching}. An application of this case is presented in the non-parametric exemplar texture synthesis algorithm proposed by Efros and Leung \cite{efros1999texture}.

% The Euclidean distance is the usual way to measure similarity between patches \cite{lebrun2013nonlocal} but many other measurements exist, corresponding to different structural properties, see Figure~\ref{fig:statistical}. We introduce $p$-norms and angle measurements similarity functions. 

% \begin{mydef}
%   \label{def:similarity_fun}
%   Let $P, Q \in \R^{\omega}$ with $\omega$ a finite domain of $\Z^2$. When it is defined we introduce
%   \begin{enumerate}[label = (\alph*)]
%   \item the $\ell^p$-similarity, $ \s{p}(P,Q) = \| P - Q \|_p = \left( \sum_{\veclet{x} \in \omega}{\vertt{P(\veclet{x}) - Q(\veclet{x})}^p}  \right)^{1/p} \eqsp , \ \text{with} \ p \in (0,+\infty) \eqsp ;$ \label{item:p}
%     \item the $\ell^{\infty}$-similarity, $s_{\infty}(P,Q) = \sup_{\omega}(|P-Q|) \eqsp ;$ \label{item:inf}
%       \item the $p$-th power of the $\ell^p$-similarity, $ \s{p,p}(P,Q) = s_{p}(P,Q)^p  \eqsp , \ \text{with} \ p \in (0,+\infty) \eqsp ;$ \label{item:p,p}
%       \item the scalar product similarity, $ \sps(P,Q) = -\langle P,Q \rangle = \frac{1}{2} \left( \s{2,2}(P,Q) - \|P\|_2^2 - \| Q \|_2^2 \right) \eqsp ;$ \label{item:ps}
%       \item the cosine similarity, $ \scos(P,Q) = \frac{\sps(P,Q)}{\| P \|_2 \|Q\|_2}, \ \text{if} \ \|P\|_2 \|Q\|_2 \neq 0 \eqsp .$ \label{item:cos}
%     \end{enumerate}
% \end{mydef}
% The locality of the measurements is ensured by the fact that these functions are defined on patches, \ie \ sub-images defined on domain $\omega$. Following conditions (1) and (3) in \cite{deledalle2012compare} we check that similarity functions \ref{item:p}, \ref{item:p,p} and \ref{item:cos} satisfy the following properties
%   \begin{itemize}[label = $\blacktriangleright$]
%   \item (Symmetry) $s(P,Q) = s(Q,P) \eqsp ;$
%   \item (Maximal self-similarity) $s(P,P) \le s(P,Q) \eqsp ;$
%   \item (Equal self-similarities) $s(P,P) = s(Q,Q) \eqsp .$
%   \end{itemize}
%  Note that since $\sps$, the scalar product similarity, is homogeneous in $P$, maximal self-similarity and equal self-similarity properties are not satisfied. In \cite{deledalle2012compare}, the authors present many other similarity functions all relying on statistical properties such as likelihood ratios, joint likelihood criteria and mutual information kernels. The latter measurement is defined by a cosine measurement in some feature space. In this paper we focus on similarity functions defined directly in the spatial domain. The limits of this restriction will be investigated in Section \ref{sec:natural_images}.


% We start by introducing structural similarity between patches and assessing some of the properties of the defined functions both for template and internal matching \cite{deledalle2012compare}. The locality of the measures is ensured by the fact that these functions are defined on patches. Let $\omega \subset \Z^2$ be an image domain. For instance $\omega$ can be a rectangular domain if we consider finite-domain images. 
% \begin{mydef}[Similarity functions]
%   Let $P$ and $Q$ be two real-valued images defined over $\omega$. A function 
%   $s : \ \R^{\omega} \times \R^{\omega} \to \R$ is called a similarity function if it satisfies the following properties:
%   \begin{itemize}[label = $\blacktriangleright$]
%   \item (Symmetry) $s(P,Q) = s(Q,P) \eqsp ;$
%   \item (Maximal self-similarity) $s(P,P) \leq s(P,Q) \eqsp ;$
%   \item (Equal self-similarities) $s(P,P) = s(Q,Q) \eqsp .$
%   \end{itemize}
% \end{mydef}
% The Euclidean distance is the usual way to measure similarity between patches \cite{lebrun2013nonlocal} but many other measurements exist, corresponding to different structural properties%, see Figure~\ref{fig:statistical}%
% . In the following examples we introduce $p$-norms and angle measurements similarity functions.
% \begin{itemize}[label = $\blacktriangleright$]
%       \item $ \s{p}(P,Q) = \| P - Q \|_p = \left( \summ{\veclet{x} \in \omega}{}{\vertt{P(\veclet{x}) - Q(\veclet{x})}^p}\right)^{\frac{1}{p}} \eqsp , \ \text{with} \ p \in (0,+\infty) \eqsp ;$
%       \item $ \s{p,p}(P,Q) = s_{p}(P,Q)^p = \summ{\veclet{x} \in \omega}{}{\vertt{P(\veclet{x}) - Q(\veclet{x})}^p} \eqsp , \ \text{with} \ p \in (0,+\infty) \eqsp ;$
%       \item $ \sps(P,Q) = -\langle P,Q \rangle = \frac{1}{2} \left( \s{2,2}(P,Q) - \|P\|_2^2 - \| Q \|_2^2 \right) \eqsp ;$
%       \item $ \scos(P,Q) = \frac{\sps(P,Q)}{\| P \|_2 \|Q\|_2}, \ \text{if} \ \|P\|_2 \|Q\|_2 \neq 0 \eqsp .$
%       \end{itemize}
%    The definition of $s_p$ can be extended to $(0,+\infty]$ by setting $s_{\infty}(P,Q) = \sup_{\omega}(|P-Q|)$.
% Note that since $\sps$, the scalar product similarity, is homogeneous in $P$, maximal self-similarity and equal self-similarity properties are not satisfied. However, on the subset of image with fixed $\ell^2$ norm $\sps$ has the same behavior as $\s{2,2}$.  In \cite{deledalle2012compare}, the authors present many other similarity functions all relying on statistical properties such as likelihood ratios, joint likelihood criteria and mutual information kernel. The latter measurement is 
% defined by a cosine in a feature space. 

% We define the auto-similarity, respectively the template similarity, as structural measurements between the sub-image defined by $\veclet{x+t}+\omega$ in $u$ and the sub-image defined by $\veclet{x}+\omega$ in $u$, respectively $v$ a template image.

We first introduce a notion of dissimilarity between patches of an input image.
\begin{mydef}[Auto-similarity]
  Let $u$ be an image defined over a domain $\Omega = \llbracket 0,M-1 \rrbracket^2 \subset \Z^2$, with $M \in \N \backslash \{ 0\}$. Let $\omega \subset \Z^2$ be a patch domain. We introduce ${P_{\omega}(u)= (\dot{u}(\veclet{y}))_{\veclet{y} \in \omega}}$ the patch at position $\omega$ in the periodic extension of $u$ to $\Z^2$, denoted by~$\dot{u}$. We define the auto-similarity with patch domain $\omega$ and offset $\veclet{t}\in \Z^2$ by
  \begin{equation}
    \autosim(u,\veclet{t},\omega) = \norm{P_{\veclet{t}+\omega}(u) - P_{\omega}(u)}_2^2 \eqsp .
  \end{equation}
  % where $s_i$ corresponds to $s_p$ with $p \in (0,+\infty]$, $s_{p,p}$ with $p \in (0,+\infty)$, $s_{sc}$ or $s_{cos}$. In the same way we define the template similarity with patch $\omega$ and offset $\veclet{t}$ by
  % \begin{equation}
  %   \templatesim_i(u,v,\veclet{t},\omega) = s_i\left(P_{\veclet{t}+\omega}(u), P_{\omega}(v) \right).
  % \end{equation}
  \label{def:autosim}
\end{mydef}
The auto-similarity computes the distance between a patch of $u$ defined on a domain $\omega$ and the patch of $u$ defined by the domain $\omega$ shifted by the offset vector $\veclet{t}$.%  whereas the template similarity uses an image $v$ as input and computes local resemblances between $u$ and $v$.

% Suppose we evaluate the scalar product auto-similarity $\autosim_{sc}(U,\veclet{t},\omega)$ with $U$ a random field. Then the expectation of the auto-similarity function depends on second-order statistics of $U$. In the template case, the expectation of $\autosim_{sc}(U,v,\veclet{t},\omega)$ depends on first-order statistics of $U$. This shows that auto-similarity and template similarity can exhibit very different statistical behaviors even for the same similarity functions.

% It is well-known that, due to the curse of dimensionality, the $\ell^2$ norm does not behave well in large-dimensional spaces and is a poor measure of structure. Thus, considering $u$ and $v$ two images, $s_2(u,v)$, the $\ell^2$ template similarity on full images, does not yield interesting information about the perceptual differences between $u$ and $v$. The template similarity $\templatesim_2(u,v,\veclet{0}, \omega)$ avoids this effect by considering patches, thus reducing the dimension of the data (if the cardinality of $\omega$, denoted $\vertt{\omega}$, is small) and also allows for fast computation of similarity mappings. Even when considering small patches there exist other limitations such as noise and outliers sensitivity or illumination dependence, see Figure \ref{fig:statistical}.
  % \captionsetup[subfigure]{labelformat=empty}
  % \begin{figure}
  %   \centering
  %   \subfloat[ $\s{2}$]{\includegraphics[width=.2\linewidth]{./img/contrast_00_L2_20_superp.png}} \hspace{0.1cm}
  %   \subfloat[$\s{1}$]{\includegraphics[width=.2\linewidth]{./img/contrast_00_L1_20_superp.png}} \hspace{0.1cm}
  %   \subfloat[$\s{\infty}$]{\includegraphics[width=.2\linewidth]{./img/contrast_00_Linfinite_20_superp.png}} \hspace{0.1cm} \\
  %   \subfloat[$\sps$]{\includegraphics[width=.2\linewidth]{./img/contrast_00_ps_20_superp.png}} \hspace{0.1cm}
  %   \subfloat[$\scos$]{\includegraphics[width=.2\linewidth]{./img/contrast_00_cos_20_superp.png}} \hspace{0.1cm}
  %   \caption{\textit{\textbf{Structural properties of similarity functions.}} Sub-images show the twenty closest matches in the $20 \times 20$ patch space for the green upper-left patch in the original image for different similarity functions. All similarity functions correctly identify the structure of the patch, \ie \ a large clear part with diagonal textures and a dark ray on the right side of the patch, except for $\s{\infty}$ which is too sensitive to outliers. Indeed outliers have more importance for $\s{\infty}$ than they have perceptually speaking. Similarities $\s{2}$ and $\s{1}$ have analogous behaviors and find correct regions. It might be noted that $\s{1}$ is more conservative as it identifies 7 main different patches and $\s{2}$ identifies eight. Similarity $\sps$ is too sensitive to contrast and, as it finds a correct patch, it gives too much importance to illumination. The behavior of $\scos$ is interesting as it avoids some of the illumination problems encountered with the scalar product. The identified regions were also found with $\s{1}$ and $\s{2}$, but with the addition of a new one.}
  %   \label{fig:statistical}
  % \end{figure}
 %   ATTENTION : CETTE EXPÉRIENCE SE TROUVE DANS RESEARCH/PATCH_SIM/PERCEPTUAL_SCRIPT
%  \captionsetup[subfigure]{labelformat=parens}
  In what follows, we introduce an \acontrario \ framework on the auto-similarity% similarity functions
  . This framework will allow us to derive an algorithm for detecting spatial redundancy in natural images.
% \subsection{A contrario framework}
\label{sec:a_contrario_framework}
In this section we fix an image domain $\Omega \subset \Z^2$ and a patch domain $\omega \subset \Omega$. We recall that our final aim is to design a criterion that will answer the following question: are two given patches similar? This criterion will be given by the comparison between the value of a dissimilarity function and a threshold $a$. We will define the threshold $a$ so that few similarities are identified in the null hypothesis model, \ie \ similarity does not occur ``just by chance''. Thus we can reformulate the initial question: is the similarity output of a dissimilarity function between two patches small enough? Or, to be more precise, how can we set the threshold $a$ in order to obtain a criterion for assessing similarity between patches?

This formulation agrees with the \acontrario \ framework \cite{desolneux2007gestalt} which states that geometrical and/or perceptual structure in an image is meaningful if it is a rare event in a background model. This general principle is sometimes called the Helmholtz principle \cite{zhu1999embedding} or the non-accidentalness principle \cite{lowe2012perceptual}. Therefore, in order to control the number of similarities identified in the background model, we study the probability density function of the auto-similarity % and template similarity
function with input random image $U$ over $\Omega$. We will denote by $\micro$ the probability distribution of $U$ over $\R^{\Omega}$, the images over $\Omega$. We will assume that $\micro$ is a microtexture model, see Definition~\ref{def:microtexture} below for a precise definition of such a model. %\ ie \ $U$ does not present long-range spatial arrangement.
% \note{To give a concrete example, in Section \ref{sec:denoising} the background model will be a standard Gaussian white noise.}
% Consequently, exhibiting repetitive structure at long-range is a rare event in a microtexture model.
We define the following significant event which encodes spatial redundancy: $\autosim(u,\veclet{t},\omega) \leq a(\veclet{t})$,
% \begin{itemize}[label = $\blacktriangleright$]
% \item auto-similarity event: $\autosim(u,\veclet{t},\omega) \leq a(\veclet{t}) \eqsp ;$
% \item template-similarity event: $\templatesim_i(u,v,\veclet{t},\omega) \leq a(\veclet{t}) \eqsp ;$
% \end{itemize}
where $a$, the threshold function, is defined over the offsets ($\veclet{t} \in \Z^2$) but also depends on other parameters such as $\omega$ or $\micro$ % or $v$
. The dependency of $a$ with respect to $\veclet{t}$ cannot be omitted. For instance, even in a Gaussian white noise $W$, the probability distribution function of $\autosim(W, \veclet{t}, \omega)$ depends on $\veclet{t}$. %The dependency of $a$ with respect to $\omega$ simply states that the threshold must scale with the size of the patch domain.
% \remark{$a$ is a function of the offset $\veclet{t}$ but might also depends on other parameters such as $\veclet{x}$, $\omega$ or $v$.}~

% \begin{mydef}[Spatial redundancy events]
%   Let $a \in \R^{\Omega}$.
%   For each offset $\veclet{t} \in \Omega$ we denote by $\autoevent_{i,\veclet{x}+\omega}(\veclet{t},a)$ the auto-similarity event at $\veclet{t}$ defined by
%   \begin{equation}
%     \autoevent_{i,\veclet{x}+\omega}(\veclet{t},a) = \left\lbrace u \in \R^{\Omega}, \autosim(u,\veclet{x},\veclet{t},\omega) \leq a(\veclet{t}) \right\rbrace.
%   \end{equation}
%   In the same way for some $\veclet{t} \in \Omega$ and $v \in \R^{\Omega}$, we denote by $\templateevent_{i, v,\veclet{x}+\omega}(\veclet{t},a)$ defined by
%   \begin{equation}
%     \templateevent_{i,v,\veclet{x}+\omega}(\veclet{t},a) = \left\lbrace u \in \R^{\Omega}, \templatesim_i(u,v,\veclet{x},\veclet{t},\omega) \leq a(\veclet{t}) \right\rbrace.
%   \end{equation}
%   \label{def:spatial_redundancy}
% \end{mydef}

The Number of False Alarms (\NFA ) is a crucial quantity in the \acontrario \ methodology.
A false alarm is defined as an occurrence of the significant event in the background model~$\micro$. We recall that in our model the significant event is patch redundancy. This test must be conducted for every possible configurations of the significant event, \ie \ in our case we test every possible offset $\veclet{t}$. The \NFA \ is then defined as the expectation of the number of false alarms over all possible configurations% , namely $\operatorname{NFA} = \sum_{\text{configuration}} \expec[\micro]{\text{false alarm}}$
. Bounding the \NFA \ ensures that the probability of identifying $k$ offsets with spatial redundancy is also bounded, see Proposition \ref{prop:a_contrario_bound}. In what follows we give the definition of the \NFA \ in the spatial redundancy context.
% It corresponds to the sum of the probabilities of the rare event under $\micro$ for all possible configurations.
% Figure \ref{fig:a_contrario_framework} illustrates this framework.
% In this paper we aim at identifying spatial structure redundancy in natural images. Following the \acontrario \ methodology we suppose that a perceptual structure can be defined as low-probability events in microtexture models.
% In Section REF we will investigate the influence of the model choice in the detection. 

\begin{mydef}[\NFA]
  Let $U \sim \micro$, where $\micro$ is a background microtexture model.
  We define the auto-similarity probability map $\autoprob$ for any $\veclet{t} \in \Omega$, $\omega \subset \Omega$ and $a \in \R^{\Omega}$ by
        \begin{equation}\autoprob(\veclet{t},\omega, a) =  \prob[0]{ \autosim(U,\veclet{t},\omega) \leq a(\veclet{t})}  \label{eq:def_autoprob} \eqsp .\end{equation}
%   In the same way we introduce the template similarity probability map $\templateprob$ for $v \in \R^{\Omega}$ by
% \[
%         \templateprob(v,\veclet{t}, \omega,a)= \prob[0]{ \templatesim_i(U,v,\veclet{t},\omega) \leq a(\veclet{t})} \eqsp .
% \]
      We define the auto-similarity expected number of false alarms $\autonfa$ by % and template similarity expected number of false alarms $\templatenfa$ by
  \begin{equation}
    \label{eq:NFA}
  \autonfa(\omega, a) = \sum_{\veclet{t} \in \Omega} \autoprob(\veclet{t}, \omega, a) \eqsp .% \qquad \text{and} \quad \templatenfa_i(v, \omega, a) = \sum_{\veclet{t} \in \Omega} \templateprob_i(v, \veclet{t}, \omega, a) \eqsp .
  \end{equation}
  \label{def:NFA}
\end{mydef}  

% \begin{mydef}[\NFA]
%   Let $u \in \R^{\Omega}$.
%   Given an offset $\veclet{t} \in \Omega$ and $a\in \R^{\Omega}$ we define the auto-similarity detection map $\autodetec_{i,\omega}(u,\veclet{t},a)$ and the auto-similarity probability map $\autoprob_{i,\omega}(\veclet{t},a)$ as
%   \begin{equation}
%     \left\lbrace
%       \al{
%         &\autodetec_{i,\omega}(u,\veclet{t},a) = \mathbb{1}_{ \autosim(u,\veclet{t},\omega) \leq a(\veclet{t})} \eqsp , \\
%         &\autoprob_{i,\omega}(\veclet{t},a) = \mathbb{E}_{\micro}\left( \autodetec_{i,\omega}(U,\veclet{t},a) \right) = \micro\left(  \autosim(U,\veclet{t},\omega) \leq a(\veclet{t}) \right) \eqsp .
%       }\right.
%   \end{equation}
%   In the same way we introduce the template similarity detection map $\templateprob_{i,v,\omega}(u,\veclet{t},a)$ and template similarity probability map $\templateprob_{i,v,\omega}(\veclet{t},a)$ for $v \in \R^{\Omega}$ as
%   \begin{equation}
%     \left\lbrace
%       \al{
%         &\templatedetec_{i,v,\omega}(u,\veclet{t},a) = \mathbb{1}_{\left\lbrace u \in \R^{\Omega}, \templatesim_i(u,v,\veclet{t},\omega) \leq a(\veclet{t}) \right\rbrace} \eqsp , \\
%         &\templateprob_{i,v,\omega}(\veclet{t},a) = \mathbb{E}_{\micro}\left( \templatedetec_{i,v,\omega}(U,\veclet{t},a) \right) = \micro\left( \templatesim_i(U,v,\veclet{t},\omega) \leq a(\veclet{t})\right) \eqsp .}\right.
%   \end{equation}
%   The \NFA \ is defined in the auto-similarity case, respectively in the template similarity case, as the sum over $\veclet{t}$ of the auto-similarity probability map, respectively the template similarity map
%   \begin{equation}
%     \operatorname{NFA} = \summ{t \in \Omega}{}{\autoprob_{i,\omega}(\veclet{t},a)} \ \text{or} \  \summ{t \in \Omega}{}{\templateprob_{i,v,\omega}(\veclet{t},a)} \eqsp .
%     \label{eq:NFA}
%   \end{equation}
%   \label{def:NFA}
% \end{mydef}  
% Let $\pi_0$ be the probability distribution function, probability distribution function, of a microtexture model. We define the internal similarity map $\mathscr{S}^{i}(u)=s(u,u) \in \R^{\Omega}$  and the associated detection map $\mathscr{D}_{a}^i(u)=\mathbb{1}_{F_{\pi_0}(\mathscr{S}^i(u)) \leq a} \in \lbrace 0,1 \rbrace^{\Omega}$ with $a>0$. The template similarity $\mathscr{S}^t$, respectively the template detection map $\mathscr{D}^t$ are defined in a same way, replacing $s(\cdot,\cdot)$ by $s(\cdot,u_0)$.
% If a property is valid for both template and internal matching the exponent will not be specified. For the sake of simplicity we omit $a$ which will be a fixed parameter.
% \end{mydef}
Note that $\autoprob(\veclet{t}, \omega, a)$ corresponds to the probability that $\omega + \veclet{t}$ is similar to $\omega$ in the background model $U$.
  For any $\veclet{t} \in \Omega$, the cumulative distribution function of the auto-similarity random variable $\autosim(U,\veclet{t},\omega)$ under $\micro$ evaluated at value $\alpha(\veclet{t})$ is given by $\autoprob(\veclet{t},\omega,\alpha(\veclet{t}))$. We denote by ${q \mapsto \autoprob^{-1}(\veclet{t},\omega,q)}$ the inverse cumulative distribution function, potentially defined by a generalized inverse ($ \autoprob^{-1}(\veclet{t},\omega,q) = \inf \{\alpha(\veclet{t}) \in \R, \ \autoprob(\veclet{t}, \omega, \alpha(\veclet{t})) \geq q \}$), of the auto-similarity random variable for a fixed offset $\veclet{t}$, with $q \in (0,1)$ a quantile. % The inverse cumulative distribution function of the template similarity function under $\micro$ is defined in the same manner.
  We now have all the tools to control the number of detected offsets in the background model.



  \begin{mydef}[Detected offset]
    Let $u \in \R^{\Omega}$ be an image, $\omega \subset \Omega$ a patch domain, and $a \in \R^{\Omega}$. An offset $\veclet{t}$ is said to be detected with respect to $a$, % , in the auto-similarity case,
    if $\autosim(u,\veclet{t}, \omega) \leq a(\veclet{t})$. % A similar definition is derived for template similarity functions given $v \in \R^{\Omega}$.
    \label{def:detec_offset}
  \end{mydef}
Note that a detected offset in $U \sim \micro$ % the background model $\micro$
corresponds to a false alarm in the \acontrario \ model. % The next proposition defines a function $a$ such that the expected number of false alarms, \ie \ the expected number of detected offsets, is controlled in the null hypothesis case.
In what follows we suppose that the cumulative distribution function of $\autosim(U,\veclet{t}, \omega)$ is invertible for every $\veclet{t} \in \Omega$. This ensures that for any $\veclet{t} \in \Omega$ and $q \in (0,1)$ we have
  \begin{equation}
    \label{eq:invertibility}
    \autoprob\left(\veclet{t}, \omega, \autoprob^{-1}\left(\veclet{t},\omega, q\right)\right) = q \eqsp .
  \end{equation}

\begin{prop}
  \label{prop:a_contrario_bound}
  Let $\operatorname{NFA}_{\text{max}} \geq 0$ and for all $\veclet{t} \in \Omega$ define $ a(\veclet{t}) = \autoprob^{-1}\left(\veclet{t}, \omega, \operatorname{NFA}_{\text{max}} / |\Omega|\right)$. We have that for any $n \in \N \without{0}$,
  \begin{equation*}
    \autonfa(\omega, a) = \operatorname{NFA}_{\text{max}} \quad \text{and} \quad \prob[0]{ \text{\quotem{at least $n$ offsets are detected in $U$}}} \leq \frac{\operatorname{NFA}_{\text{max}}}{n} \eqsp.
  \end{equation*}
  % \begin{enumerate}[label =(\alph*)]
  % \item $\autonfa(\omega, a) = \operatorname{NFA}_{\text{max}}$. 
  % \item In addition, we have that for any $n \in \N \without{0}$
  % \[ \prob[0]{ \text{\quotem{at least $n$ offsets are detected in $U$}}} \leq \frac{\operatorname{NFA}_{\text{max}}}{n} \eqsp.\]

  % \end{enumerate}

  % In the template similarity case the same proposition holds if we replace $\autoprob(\veclet{t},\omega,a)$ by $\templateprob(v,\veclet{t},\omega,a)$.
\end{prop}
\begin{proof}
  % \begin{enumerate}[label=(\alph*)]
  %   \item
  % The proof is done in the auto-similarity case and adapts to the template similarity framework. 
  Using \eqref{eq:NFA}, and $a(\veclet{t}) = \autoprob^{-1}\left(\veclet{t}, \omega, \operatorname{NFA}_{\text{max}} / |\Omega|\right)$, we get
  \[ \autonfa(\omega, a) = \summ{\veclet{t} \in \Omega}{}{\autoprob(\veclet{t},\omega, a)} = \summ{\veclet{t} \in \Omega}{}{\autoprob\left(\veclet{t}, \omega, \autoprob^{-1}\left(\veclet{t},\omega, \operatorname{NFA}_{\text{max}} / \vertt{\Omega}\right)\right)} = \operatorname{NFA}_{\text{max}} \eqsp ,
  \]
  where the last equality is obtained using \eqref{eq:invertibility}.
  % \item 
    Concerning the upper-bound, we have, using the Markov inequality and \eqref{eq:def_autoprob}, for any $n \in \N \without{0}$
\begin{align*}
    \prob[0]{ \text{\quotem{\small at least $n$ offsets are detected in $U$}}} &= \prob[0]{\sum_{\veclet{t} \in \Omega}{}{\mathbb{1}_{\autosim(U, \veclet{t}, \omega) \leq a(\veclet{t})}} \ge n} \\ &\leq \frac{\sum_{\veclet{t} \in \Omega}{}{\expec{\mathbb{1}_{\autosim(U, \veclet{t}, \omega) \leq a(\veclet{t})}}}}{n}  \leq \frac{\operatorname{NFA}_{\text{max}}}{n} \eqsp ,
\end{align*}
where $\mathbb{1}_{\autosim(U, \veclet{t}, \omega) \leq a(\veclet{t})} = 1$ if $\autosim(U, \veclet{t}, \omega) \leq a(\veclet{t})$ and $0$ otherwise.
%  \end{enumerate}
  % First let us remark that $\mathbb{1}_{F_{\pi_0}(\mathscr{S}(u)) \leq a} = \mathbb{1}_{\mathscr{S}(u) \leq F_{\pi_0}^{-1}(a)}$ where $F_{\pi_0}$ is the cumulative distribution function, cumulative distribution function, of the similarity distribution function under the microtexture model. Using this equality we obtain
  % \[ \al{
  %   P_{\veclet{u} \sim \pi_0}\left( \mathscr{N}_a(\veclet{u}) \ge \alpha \right) &\leq \frac{E(\mathscr{N}_a(\veclet{u}))}{\alpha}. \\
  %   &\leq \frac{E \left( \summ{x \in \Omega}{}{\mathbb{1}_{s(\veclet{u},\veclet{u}) \leq F_{\pi_0}^{-1}(a)}}\right)}{\alpha} \\
  %   &\leq \frac{\vertt{\Omega} F_{\pi_0}^{-1}(a)}{\alpha}.
  % }\]
\end{proof}

Thus, setting $a$ as in Proposition \ref{prop:a_contrario_bound}, we have that an offset $\veclet{t} \in \Omega$ is detected for an image~$u \in \R^{\Omega}$ if%, \ie \ corresponds to spatial redundancy, for a given \NFAmax \ if
\begin{equation}\autosim(u,\veclet{t},\omega) \leq \autoprob^{-1}\left(\veclet{t},\omega, \operatorname{NFA}_{\text{max}} / \vertt{\Omega}\right) \eqsp . \label{eq:icdf_ineq}\end{equation}
This \acontrario \ detection framework % , see Figure \ref{fig:a_contrario_framework},
can then be simply rewritten as 1) computing the auto-similarity function with input image $u$, 2) thresholding the obtained dissimilarity map with the inverse cumulative distribution function of the computed dissimilarity function under $\micro$. % The choice of $\micro$ will be discussed in the next section.
The computed threshold depends on the offset and Proposition \ref{prop:a_contrario_bound} ensures probabilistic guarantees on the expected number of detections under $\micro$. % In many cases, cumulative distribution function of similarity functions are easier to compute than inverse cumulative distribution function.
Using the inverse property of the inverse cumulative distribution function and \eqref{eq:icdf_ineq}, we obtain that an offset is detected if and only if
\begin{equation}\prob[0]{\autosim(U,\veclet{t},\omega) \leq \autosim(u,\veclet{t},\omega)}=  \autoprob\left(\veclet{t}, \omega, \autosim(u,\veclet{t},\omega)\right) \leq \operatorname{NFA}_{\text{max}} /\vertt{\Omega} \eqsp . \label{eq:true_detec}\end{equation}
Therefore, the thresholding operation can be conducted either on $\autosim(u,\veclet{t}, \omega)$, see \eqref{eq:icdf_ineq}, or on $\autoprob\left(\veclet{t}, \omega, \autosim(u,\veclet{t},\omega)\right)$, see \eqref{eq:true_detec}.
This property will be used in Section \ref{sec:detection-algorithm} to define a similarity detection algorithm based on the evaluation of $\autosim(u,\veclet{t}, \omega)$.% the auto-similarity. % associated to the square $\ell^2$ norm, see Algorithm~\ref{alg:auto-similaritydetection}.
% \begin{figure}
%   \centering
%   \input{a_contrario_framework.tex}
%   \caption{\figuretitle{A contrario methodology} For structure detection purposes this detection is accomplished on parallel on every pixel of the image. The event $\mathcal{E}$ corresponds to the auto-similarity or the template similarity event described in this section and encoded in $\left\lbrace u \in \R^{\Omega}, \autosim(u,\veclet{t},\omega) \leq a(\veclet{t}) \right\rbrace$. The output of the \acontrario \ methodology is a binary map over $\Omega$ such that for any offset $\veclet{t}$ we associate 1 if the offset is detected and 0 otherwise. It expresses the significativity decision for every possible offset.}
%   \label{fig:a_contrario_framework}
% \end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_v3"
%%% End:

